EMBERS at 4 years: Experiences operating an Open Source Indicators Forecasting System

EMBERS is an anticipatory intelligence system forecasting population-level events in multiple countries of Latin America. A deployed system from 2012, EMBERS has been generating alerts 24x7 by ingesting a broad range of data sources including news, blogs, tweets, machine coded events, currency rates, and food prices. In this paper, we describe our experiences operating EMBERS continuously for nearly 4 years, with specific attention to the discoveries it has enabled, correct as well as missed forecasts, and lessons learnt from participating in a forecasting tournament including our perspectives on the limits of forecasting and ethical considerations.

==> figures/narrative.tex <==
\begin{figure} %[!t]
    \centering
    \fbox{
\begin{minipage}{\columnwidth}{
EMBERS forecasts that there will be a {\color{red}violent} protest on
{\color{red}February, 18th 2014}
in {\color{red}Caracas}, the {\color{red}capital city of Venezuela}.
We predict that the protest will involve
people working in the {\color{red}business sector}. The protest will be related to
{\color{red}discontent about economic policies}.
\\
There were {\color{blue}5, 5, and 5 other similar
warnings in last 2, 7 and 30 days}, respectively.
\\
The forecast date of the warning falls in {\color{blue}week 7}, which
{\color{blue}may have historical
importance}; this {\color{blue}week is found to be statistically significant}
(pval=0.00461919415894, zscore=2.832, avg. count=57.25, mean=21.569 +/- 12.597)
\\
Audit trail of the warning includes an {\color{blue}article printed 2014-02-17}.
\\
\underline{Major players} involved in the protest include {\color{red}Venezuelan opposition leader, students,
President Nicolas Maduro, and Leopoldo Lopez}.
\\
\underline{Reasons}: Protest {\color{magenta}against rising
inflation and crime}; Protestors want a {\color{magenta}political change}; President Nicolas
Maduro has {\color{magenta} accused US consular officials} and {\color{magenta}right-wing}.
\\
\underline{Protests are characterized by}: Venezuelan opposition leader
spearheaded days of protest and {\color{green}calling for peaceful
demonstration}; Maduro accused official on {\color{red} 2014-12-16}; Protests
have seen {\color{green}several deadly street protests}; Three people were
{\color{green}killed on} {\color{red}2014-02-12}; {\color{green}Demonstrations}
setting days of clashes; {\color{green}supporters to march to}
{\color{red}Interior Ministry} {\color{green}on} {\color{red}2014-02-18}.
}
\end{minipage}
}
    \caption{An example narrative for a EMBERS alert message. Here, color
{\color{red}red} indicates named entities, {\color{green} green} refers to
descriptive protest related keywords. Items in {\color{blue} blue} are historical or
real time statistics and those in {\color{magenta}magenta} refer
to inferred reasons of protest. }
    \label{fig:narrative}
\vspace{-5mm}
\end{figure}

